Towards Few-shot Entity Recognition in Document Images: A Label-aware Sequence-to-Sequence Framework

Entity recognition is a fundamental task in understanding document images. Traditional sequence labeling frameworks treat the entity types as class IDs and rely on extensive data and high-quality annotations to learn semantics which are typically expensive in practice. In this paper, we aim to build an entity recognition model requiring only a few shots of annotated document images. To overcome the data limitation, we propose to leverage the label surface names to better inform the model of the target entity type semantics and also embed the labels into the spatial embedding space to capture the spatial correspondence between regions and labels. Specifically, we go beyond sequence labeling and develop a novel label-aware seq2seq framework, LASER. The proposed model follows a new labeling scheme that generates the label surface names word-by-word explicitly after generating the entities. During training, LASER refines the label semantics by updating the label surface name representations and also strengthens the label-region correlation. In this way, LASER recognizes the entities from document images through both semantic and layout correspondence. Extensive experiments on two benchmark datasets demonstrate the superiority of LASER under the few-shot setting.

==> src/tab1-result_full.tex <==
\begin{table*}[t]
    \centering
    \caption{Evaluation Results with Different Sizes of Few-shot Training Samples: \textbf{Bold} denotes the best model; \underline{Underline} denotes the second-best model. 
    % \jingbo{I don't think we need to make \MODEL bold?} \jingbo{maybe we should put our \MODEL together with other baselines in one section and leave the ablation below it as a separate section in the table. currently, baselines are in the same section and our methods are in one section. Then, when marking the second best, we can focus on the baselines but not our ablation?}
    }
    \label{tab:main}%
    % \vspace{-3mm}
\small
\setlength{\tabcolsep}{8pt}
\begin{tabular}{clcccccc}
\toprule
\multirow{2}[4]{*}{$|\mathcal{P}|$} & \multirow{2}[4]{*}{\textbf{Model}} & \multicolumn{3}{c}{\textbf{FUNSD}} & \multicolumn{3}{c}{\textbf{CORD-Lv1}} \\
\cmidrule{3-8}      &       & \textbf{Precision} & \textbf{Recall} & \textbf{F-1} & \textbf{Precision} & \textbf{Recall} & \textbf{F-1} \\
\midrule
\multirow{8}[4]{*}{1} & BERT  & 9.62$\pm$2.24 & 24.14$\pm$3.46 & 13.55$\pm$2.09 & 30.64$\pm$2.80 & 45.60$\pm$3.45 & 36.64$\pm$3.10 \\
      & RoBERTa & 9.29$\pm$1.57 & 22.06$\pm$5.64 & 12.76$\pm$1.91 & 30.66$\pm$4.25 & 44.39$\pm$6.72 & 36.25$\pm$5.18 \\
      & LayoutLM & \underline{11.39$\pm$1.12} & \underline{24.73$\pm$7.38} & \underline{15.18$\pm$2.17} & \underline{33.27$\pm$7.32} & \textbf{49.49$\pm$10.26} & \underline{39.77$\pm$8.47} \\
      & LayoutReader & 11.32$\pm$0.62 & 22.53$\pm$4.80 & 14.84$\pm$1.25 & 32.17$\pm$4.64 & \underline{45.61$\pm$6.54} & 37.70$\pm$5.31 \\
      & LASER & \textbf{30.40$\pm$4.89} & \textbf{35.20$\pm$7.20} & \textbf{32.36$\pm$5.14} & \textbf{47.63$\pm$3.90} & 45.52$\pm$5.84 & \textbf{46.24$\pm$3.01} \\
\cmidrule{2-8}      & \textit{(IRLVT)} & 30.64$\pm$5.89 & 33.45$\pm$9.14 & 31.62$\pm$6.61 & 48.57$\pm$4.93 & 44.12$\pm$6.36 & 45.84$\pm$3.57 \\
      & \textit{(Sub1)} & 31.78$\pm$4.75 & 34.21$\pm$7.44 & 32.66$\pm$5.10 & 48.12$\pm$4.15 & 48.47$\pm$6.60 & 48.04$\pm$4.06 \\
      & \textit{(Sub2)} & 30.90$\pm$5.20 & 35.97$\pm$8.57 & 33.03$\pm$6.31 & 45.59$\pm$5.68 & 44.09$\pm$7.87 & 44.38$\pm$5.39 \\
\midrule
\multirow{8}[4]{*}{3} & BERT  & 16.42$\pm$4.30 & 34.74$\pm$5.36 & 22.19$\pm$5.05 & 39.62$\pm$3.99 & 56.65$\pm$4.03 & 46.58$\pm$3.94 \\
      & RoBERTa & 16.71$\pm$3.63 & 31.28$\pm$3.55 & 21.66$\pm$3.84 & 44.51$\pm$4.69 & 60.18$\pm$4.69 & 51.15$\pm$4.70 \\
      & LayoutLM & \underline{28.67$\pm$6.56} & \textbf{47.22$\pm$8.31} & \underline{35.42$\pm$7.00} & \underline{47.68$\pm$7.49} & \textbf{63.93$\pm$7.04} & \underline{54.57$\pm$7.46} \\
      & LayoutReader & 22.37$\pm$2.03 & 35.19$\pm$4.97 & 27.19$\pm$2.56 & 43.85$\pm$4.72 & 56.90$\pm$2.47 & 49.47$\pm$3.95 \\
      & LASER & \textbf{43.66$\pm$1.97} & \underline{47.08$\pm$5.72} & \textbf{45.21$\pm$3.74} & \textbf{61.16$\pm$3.11} & \underline{60.33$\pm$5.65} & \textbf{60.63$\pm$4.00} \\
\cmidrule{2-8}      & \textit{(IRLVT)} & 43.51$\pm$1.46 & 47.92$\pm$5.93 & 45.44$\pm$3.36 & 61.50$\pm$2.52 & 59.17$\pm$4.11 & 60.27$\pm$2.99 \\
      & \textit{(Sub1)} & 43.87$\pm$1.33 & 47.11$\pm$6.07 & 45.26$\pm$3.44 & 61.54$\pm$2.76 & 58.79$\pm$6.76 & 60.00$\pm$4.57 \\
      & \textit{(Sub2)} & 43.88$\pm$1.34 & 48.01$\pm$6.86 & 45.65$\pm$3.93 & 61.85$\pm$2.16 & 60.29$\pm$2.85 & 61.03$\pm$2.10 \\
\midrule
\multirow{8}[4]{*}{5} & BERT  & 20.57$\pm$2.59 & 39.25$\pm$1.10 & 26.93$\pm$2.46 & 45.73$\pm$4.31 & 63.29$\pm$3.68 & 53.06$\pm$4.14 \\
      & RoBERTa & 19.47$\pm$2.32 & 35.04$\pm$1.89 & 24.94$\pm$1.93 & 52.21$\pm$4.55 & \underline{66.63$\pm$5.52} & 58.54$\pm$4.92 \\
      & LayoutLM & \underline{39.24$\pm$4.33} & \textbf{58.20$\pm$2.45} & \underline{46.72$\pm$3.12} & \underline{56.13$\pm$7.39} & \textbf{71.66$\pm$6.13} & \underline{62.91$\pm$7.04} \\
      & LayoutReader & 27.52$\pm$3.44 & 41.17$\pm$4.01 & 32.89$\pm$3.28 & 51.97$\pm$8.42 & 63.82$\pm$7.87 & 57.24$\pm$8.32 \\
      & LASER & \textbf{47.25$\pm$1.93} & \underline{52.85$\pm$1.22} & \textbf{49.87$\pm$1.29} & \textbf{65.62$\pm$3.79} & 64.90$\pm$5.78 & \textbf{65.23$\pm$4.70} \\
\cmidrule{2-8}      & \textit{(IRLVT)} & 46.94$\pm$1.87 & 52.96$\pm$2.03 & 49.74$\pm$1.63 & 63.67$\pm$3.82 & 61.10$\pm$5.21 & 62.33$\pm$4.48 \\
      & \textit{(Sub1)} & 47.43$\pm$2.29 & 52.19$\pm$2.09 & 49.68$\pm$1.98 & 65.05$\pm$5.59 & 63.64$\pm$7.16 & 64.31$\pm$6.34 \\
      & \textit{(Sub2)} & 47.46$\pm$2.18 & 53.50$\pm$1.01 & 50.26$\pm$1.16 & 65.57$\pm$3.04 & 64.71$\pm$3.97 & 65.12$\pm$3.38 \\
\midrule
\multirow{8}[4]{*}{7} & BERT  & 21.44$\pm$2.07 & 40.87$\pm$3.79 & 28.09$\pm$2.48 & 50.13$\pm$4.35 & 66.67$\pm$3.67 & 57.20$\pm$4.07 \\
      & RoBERTa & 23.68$\pm$3.06 & 38.74$\pm$3.54 & 29.32$\pm$3.08 & 55.14$\pm$4.49 & \underline{69.35$\pm$4.16} & 61.43$\pm$4.42 \\
      & LayoutLM & \underline{43.23$\pm$5.27} & \textbf{61.73$\pm$5.97} & \underline{50.76$\pm$5.30} & \underline{62.87$\pm$3.98} & \textbf{76.38$\pm$2.72} & \textbf{68.96$\pm$3.49} \\
      & LayoutReader & 31.22$\pm$3.14 & 45.08$\pm$3.83 & 36.85$\pm$3.26 & 54.43$\pm$5.89 & 65.48$\pm$5.34 & 59.42$\pm$5.68 \\
      & LASER & \textbf{50.62$\pm$3.26} & \underline{53.63$\pm$2.89} & \textbf{51.98$\pm$2.00} & \textbf{68.02$\pm$3.16} & 66.87$\pm$4.82 & \underline{67.40$\pm$3.76} \\
\cmidrule{2-8}      & \textit{(IRLVT)} & 50.30$\pm$2.26 & 54.14$\pm$3.48 & 52.08$\pm$2.26 & 66.08$\pm$3.26 & 64.73$\pm$5.08 & 65.32$\pm$3.74 \\
      & \textit{(Sub1)} & 50.22$\pm$3.20 & 53.79$\pm$3.13 & 51.88$\pm$2.56 & 67.61$\pm$4.19 & 66.64$\pm$5.72 & 67.08$\pm$4.72 \\
      & \textit{(Sub2)} & 50.43$\pm$2.88 & 54.03$\pm$2.71 & 52.10$\pm$2.09 & 66.64$\pm$3.97 & 63.59$\pm$7.00 & 65.02$\pm$5.47 \\
\bottomrule
\end{tabular}%
% \vspace{-3mm}
\end{table*}%

==> src/tab2-funsd_unk.tex <==
% Table generated by Excel2LaTeX from sheet 'diff-tag'
\begin{table}[t]
  \centering
  \caption{Ablation Study: {IRLVT} uses the irrelevant tokens, [\textit{x}, \textit{y}, \textit{z}], as labels; {ORIG} uses the original label surface names; {Sub1} uses [\textit{title}, \textit{key}, \textit{value}] as substitutes; {Sub2} uses [\textit{page}, \textit{topic}, \textit{value}] as substitutes. 
%   \jingbo{use textit for those label surface names.}
\textbf{Bold} denotes the best model; \underline{Underline} denotes the second-best model.
% \jingbo{We probably don't need to mention the surface names every time. Move these to the caption here so we can make this table fit in one column.}
}
  \label{tab:unk1}%
%   \vspace{-3mm}
% \scalebox{0.8}{
  \small
% Table generated by Excel2LaTeX from sheet 'diff-tag'
\setlength{\tabcolsep}{1.2mm}{
% Table generated by Excel2LaTeX from sheet 'FUNSD-Better'
% Table generated by Excel2LaTeX from sheet 'FUNSD-Better'
\begin{tabular}{clccc}
    \toprule
    \multirow{2}[4]{*}{$|\mathcal{P}|$} & \multirow{2}[4]{*}{\textbf{Label}} & \multicolumn{3}{c}{\textbf{FUNSD}} \\
    \cmidrule{3-5}      &       & \textbf{Precision} & \textbf{Recall} & \textbf{F-1} \\
    \midrule
    \multirow{4}[4]{*}{1} & IRLVT & 30.64$\pm$5.89 & 33.45$\pm$9.14 & 31.62$\pm$6.61 \\
          & ORIG & 30.40$\pm$4.89 & \underline{35.20$\pm$7.20} & 32.36$\pm$5.14 \\
    \cmidrule{2-5}      & Sub1  & \textbf{31.78$\pm$4.75} & 34.21$\pm$7.44 & \underline{32.66$\pm$5.10} \\
          & Sub2  & \underline{30.90$\pm$5.20} & \textbf{35.97$\pm$8.57} & \textbf{33.03$\pm$6.31} \\
    \midrule
    \multirow{4}[4]{*}{3} & IRLVT & 43.51$\pm$1.46 & \underline{47.92$\pm$5.93} & \underline{45.44$\pm$3.36} \\
          & ORIG & 43.66$\pm$1.97 & 47.08$\pm$5.72 & 45.21$\pm$3.74 \\
    \cmidrule{2-5}      & Sub1  & \underline{43.87$\pm$1.33} & 47.11$\pm$6.07 & 45.26$\pm$3.44 \\
          & Sub2  & \textbf{43.88$\pm$1.34} & \textbf{48.01$\pm$6.86} & \textbf{45.65$\pm$3.93} \\
    \midrule
    \multirow{4}[4]{*}{5} & IRLVT & 46.94$\pm$1.87 & \underline{52.96$\pm$2.03} & 49.74$\pm$1.63 \\
          & ORIG & 47.25$\pm$1.93 & 52.85$\pm$1.22 & \underline{49.87$\pm$1.29} \\
    \cmidrule{2-5}      & Sub1  & \underline{47.43$\pm$2.29} & 52.19$\pm$2.09 & 49.68$\pm$1.98 \\
          & Sub2  & \textbf{47.46$\pm$2.18} & \textbf{53.50$\pm$1.01} & \textbf{50.26$\pm$1.16} \\
    \midrule
    \multirow{4}[4]{*}{7} & IRLVT & 50.30$\pm$2.26 & \textbf{54.14$\pm$3.48} & \underline{52.08$\pm$2.26} \\
          & ORIG & \textbf{50.62$\pm$3.26} & 53.63$\pm$2.89 & 51.98$\pm$2.00 \\
    \cmidrule{2-5}      & Sub1  & 50.22$\pm$3.20 & 53.79$\pm$3.13 & 51.88$\pm$2.56 \\
          & Sub2  & \underline{50.43$\pm$2.88} & \underline{54.03$\pm$2.71} & \textbf{52.10$\pm$2.09} \\
    \bottomrule
    \end{tabular}%
% \vspace{-3mm}
% }
}
\end{table}%

==> src/tab3-cord_unk.tex <==
% Table generated by Excel2LaTeX from sheet 'diff-tag'
\begin{table}[t]
  \centering
  \caption{Ablation Study: {IRLVT} uses the irrelevant tokens, [\textit{w}, \textit{x}, \textit{y}, \textit{z}], as labels; {ORIG} uses the original label surface names; {Sub1} uses [\textit{info}, \textit{etc}, \textit{small}, \textit{number}] as substitutes; {Sub2} uses [\textit{page}, \textit{non}, \textit{part}, \textit{price}] as substitutes. 
%   \jingbo{use textit for those label surface names.}
\textbf{Bold} denotes the best model; \underline{Underline} denotes the second-best model.
% \jingbo{We probably don't need to mention the surface names every time. Move these to the caption here so we can make this table fit in one column.}
}
  \label{tab:unk2}%
%   \vspace{-3mm}
% \scalebox{0.8}{
  \small
% Table generated by Excel2LaTeX from sheet 'diff-tag'
\setlength{\tabcolsep}{1.2mm}{
% Table generated by Excel2LaTeX from sheet 'CORD-Better'
% Table generated by Excel2LaTeX from sheet 'CORD-Better'
\begin{tabular}{clccc}
    \toprule
    \multirow{2}[4]{*}{$|\mathcal{P}|$} & \multirow{2}[4]{*}{\textbf{Label}} & \multicolumn{3}{c}{\textbf{CORD-Lv1}} \\
    \cmidrule{3-5}      &       & \textbf{Precision} & \textbf{Recall} & \textbf{F-1} \\
    \midrule
    \multirow{4}[4]{*}{1} & (IRLVT) & \textbf{48.57$\pm$4.93} & 44.12$\pm$6.36 & 45.84$\pm$3.57 \\
          & LASER & 47.63$\pm$3.90 & \underline{45.52$\pm$5.84} & \underline{46.24$\pm$3.01} \\
    \cmidrule{2-5}      & Sub1  & \underline{48.12$\pm$4.15} & \textbf{48.47$\pm$6.60} & \textbf{48.04$\pm$4.06} \\
          & Sub2  & 45.59$\pm$5.68 & 44.09$\pm$7.87 & 44.38$\pm$5.39 \\
    \midrule
    \multirow{4}[4]{*}{3} & (IRLVT) & 61.50$\pm$2.52 & 59.17$\pm$4.11 & 60.27$\pm$2.99 \\
          & LASER & 61.16$\pm$3.11 & \textbf{60.33$\pm$5.65} & \underline{60.63$\pm$4.00} \\
    \cmidrule{2-5}      & Sub1  & \underline{61.54$\pm$2.76} & 58.79$\pm$6.76 & 60.00$\pm$4.57 \\
          & Sub2  & \textbf{61.85$\pm$2.16} & \underline{60.29$\pm$2.85} & \textbf{61.03$\pm$2.10} \\
    \midrule
    \multirow{4}[4]{*}{5} & (IRLVT) & 63.67$\pm$3.82 & 61.10$\pm$5.21 & 62.33$\pm$4.48 \\
          & LASER & \textbf{65.62$\pm$3.79} & \textbf{64.90$\pm$5.78} & \textbf{65.23$\pm$4.70} \\
    \cmidrule{2-5}      & Sub1  & 65.05$\pm$5.59 & 63.64$\pm$7.16 & 64.31$\pm$6.34 \\
          & Sub2  & \underline{65.57$\pm$3.04} & \underline{64.71$\pm$3.97} & \underline{65.12$\pm$3.38} \\
    \midrule
    \multirow{4}[4]{*}{7} & (IRLVT) & 66.08$\pm$3.26 & 64.73$\pm$5.08 & 65.32$\pm$3.74 \\
          & LASER & \textbf{68.02$\pm$3.16} & \textbf{66.87$\pm$4.82} & \textbf{67.40$\pm$3.76} \\
    \cmidrule{2-5}      & Sub1  & \underline{67.61$\pm$4.19} & \underline{66.64$\pm$5.72} & \underline{67.08$\pm$4.72} \\
          & Sub2  & 66.64$\pm$3.97 & 63.59$\pm$7.00 & 65.02$\pm$5.47 \\
    \bottomrule
    \end{tabular}%
% \vspace{-3mm}
% }
}
\end{table}%
